Trends, Challenges and Adopted Strategies in RoboCup@Home (2019 version)

Scientific competitions are crucial in the field of service robotics. They foster knowledge exchange and benchmarking, allowing teams to test their research in unstandardized scenarios. In this paper, we summarize the trending solutions and approaches used in RoboCup@Home. Further on, we discuss the attained achievements and challenges to overcome in relation with the progress required to fulfill the long-term goal of the league. Consequently, we propose a set of milestones for upcoming competitions by considering the current capabilities of the robots and their limitations. With this work we aim at laying the foundations towards the creation of roadmaps that can help to direct efforts in testing and benchmarking in robotics competitions.

==> setup/acknowledgements.tex <==
% If you'd like to thank anyone, place your comments here
% \begin{acknowledgements}
% \end{acknowledgements}
